Variance and covariance of distributions on graphs

We develop a theory to measure the variance and covariance of probability distributions defined on the nodes of a graph, which takes into account the distance between nodes. Our approach generalizes the usual (co)variance to the setting of weighted graphs and retains many of its intuitive and desired properties. Interestingly, we find that a number of famous concepts in graph theory and network science can be reinterpreted in this setting as variances and covariances of particular distributions. As a particular application, we define the maximum variance problem on graphs with respect to the effective resistance distance, and characterize the solutions to this problem both numerically and theoretically. We show how the maximum variance distribution is concentrated on the boundary of the graph, and illustrate this in the case of random geometric graphs. Our theoretical results are supported by a number of experiments on a network of mathematical concepts, where we use the variance and covariance as analytical tools to study the (co-)occurrence of concepts in scientific papers with respect to the (network) relations between these concepts.

==> shared.tex <==
% Not in the template %%%%%%%%
% Used for creating new theorem and remark environments

% Packages & Macros (krl)
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{xcolor} %to color comments
\usepackage{bbm} %to use indicator function
\usepackage{float} %to use [h!] with figures
\usepackage{amsopn} %standard?
\usepackage{mathrsfs} %for \mathscr
\usepackage{comment} %to comment out sections
\usepackage{tabularx} %to fit tables to page width


\renewcommand{\Pr}{\operatorname{Pr}}
\newcommand{\var}{\operatorname{var}}
\newcommand{\cov}{\operatorname{cov}}
\newcommand{\corr}{\operatorname{corr}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\divg}{\operatorname{div}}
\newcommand{\argmax}{\operatorname{argmax}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%to include code block
\usepackage{listings}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Variance and covariance of distributions on graphs}{K. Devriendt, S. Martin-Guttierez, and R. Lambiotte}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Variance and covariance of distributions on graphs\thanks{Accepted for publication in SIAM Review, Research Spotlights
\funding{
KD was supported by The Alan Turing Institute under the EPSRC grant EP/N510129/1. SMG acknowledges support by the Spanish Ministry of Science, Innovation and Universities (MICIU) under Contract No. PGC2018-093854-B-I00 and Spanish Ministry of Education, Culture and Sport (Grant No. FPU15/01461).}}}

\author{Karel Devriendt\thanks{Mathematical Institute, University of Oxford, Oxford, UK and The Alan Turing Institute, London, UK
  (\email{karel.devriendt@maths.ox.ac.uk})}
\and Samuel Martin-Gutierrez\thanks{Grupo de Sistemas Complejos, Universidad Polit\'{e}cnico de Madrid, Madrid, Spain and Complexity Science Hub Vienna, Wien, Austria
  }
\and Renaud Lambiotte\thanks{Mathematical Institute, University of Oxford, Oxford, UK}}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

